OntoSeer -- A Recommendation System to Improve the Quality of Ontologies

Building an ontology is not only a time-consuming process, but it is also confusing, especially for beginners and the inexperienced. Although ontology developers can take the help of domain experts in building an ontology, they are not readily available in several cases for a variety of reasons. Ontology developers have to grapple with several questions related to the choice of classes, properties, and the axioms that should be included. Apart from this, there are aspects such as modularity and reusability that should be taken care of. From among the thousands of publicly available ontologies and vocabularies in repositories such as Linked Open Vocabularies (LOV) and BioPortal, it is hard to know the terms (classes and properties) that can be reused in the development of an ontology. A similar problem exists in implementing the right set of ontology design patterns (ODPs) from among the several available. Generally, ontology developers make use of their experience in handling these issues, and the inexperienced ones have a hard time. In order to bridge this gap, we propose a tool named OntoSeer, that monitors the ontology development process and provides suggestions in real-time to improve the quality of the ontology under development. It can provide suggestions on the naming conventions to follow, vocabulary to reuse, ODPs to implement, and axioms to be added to the ontology. OntoSeer has been implemented as a Prot\'eg\'e plug-in.

==> OntoSeer - A Recommendation System to Improve the Quality of Ontologies /files/Conclusion.tex <==
\section{Conclusion and Future Work}

Developing an ontology is often confusing and time consuming, especially for the inexperienced developers. They have many choices to make, such as the classes and properties to create or reuse, ODPs to use, the different axioms to include in the ontology and the naming conventions to follow. We developed a Prot\'eg\'e plugin named OntoSeer to ease the process of building an ontology. Our tool recommends classes, properties, axioms, and ontology design patterns in real-time while a user is developing the ontology. We have conducted a user study of the tool. There were 21 respondents. Almost all the users are satisfied with the recommendations provided by OntoSeer. The majority of the users (14 out of 21) said that OntoSeer also helps them in saving modelling time. In our evaluation, we also show that the recommendations generated by OntoSeer are relevant and are of good quality. In the future, we plan to engage in a dialogue with the ontology developer in real-time to resolve confusing issues such as a term being a class vs. a property vs. an instance. A dialogue with the user also helps in checking whether the ontology can answer the competency questions.

\textbf{Acknowledgement.} This work has partially been supported by the Infosys Centre for Artificial Intelligence (CAI), IIIT-Delhi, India.

%According to 68\% percent of users, it is helpful to them, and 66.67\%of users agree that it saves their modelling time. Users were happy with how accurate the axiom recommendation was with minimal input.

 %This confusion will be resolved by asking the ontology developer a series of questions related to the interaction of the term with other classes, the possible instances it can have, etc. A dialogue with the user also helps in checking whether the ontology helps in answering the competency questions and if it does not, provide appropriate recommendations to improve the ontology and answer the competency questions. We are also planning to provide a spell-check of the terms to the user and recommend terms similar to the term but with a correct spelling. 

%Thus if a user builds a class named ``acicul", Ontoseer will recommend alternate names such as ``acicula", ``aciculae", ``auriculae". 

% along with the recommendation of axioms that are not present in the already built ontology.

%\section{Conclusion}

%Building good ontologies is a challenging and confusing task even for a domain expert if they are not proficient in logic.Good ontology has been defined as the one that serves its intended purpose thoroughly,\cite{hitzler_foundations_2010},that is, a good ontology is the one that infers the knowledge one wants to capture from it.

%Over time researchers have developed some evaluating criteria for ontologies to qualify as good ontology.

%\textbf{Logical Criteria:}One of the basic evaluation criteria,it comprises of the evaluation of ontology based on whether there is at least one model where all the axioms of the ontology holds. If there does not exist any such models ,that means the ontology is \textit{inconsistent} or \textit{unsatisfiable}.In general an inconsistent ontology occurs due to some modelling errors.

%Some of the commonly made modelling errors which make the ontology inconsistent are:

%\textbf{Missing Disjointness}:This is one of the commonly made logical mistake.Class "Living Being" and Class "Non Living Being" are disjoint classes ,they cannot share instances but one needs to explicitly mention that while designing the model\cite{poveda-villalon_oops!_2014}\cite{rector_owl_2004}\cite{gomez-perez_ontology_2004}. 

%\textbf{Namespace Hijacking}: Trying to access terms not defined in the current namespace but from other namespaces.This logical pitfall is related to publishing Linked data \cite{heath_linked_2011}\cite{poveda-villalon_oops!_2014}.

%\textbf{Untyped Class and Untyped Property}: Sometimes a resource is being used as a class or a property without explicitly defining them as  \textit{rdfs:class} or\textit{rdf:Property}.For example instances has been included for a resource without defining it as a Class is another type of commonly made logical mistake\cite{hogan_weaving_2010}\cite{poveda-villalon_oops!_2014}.


%\textbf{Structural and Formal Criteria:}To maintain the quality of ontology it is preferable that the ontology should not be containing more than one semantically equivalent classes.Otherwise it is indicative of some design flaws in the ontology.\\
%    For example: Dog $\sqsubseteq$ Mammal ;
%                 Mammal $\sqsubseteq$ Person;
%                 Person $\sqsubseteq$ Dog\\
%Now from this circular chain all of Dog ,Mammal, Person all are same which does not conform to the real world scenario.
%  Missing requirements:The ORSD(Ontology requirement Specification Document) have some requirements based on which an ontology is designed.Anything missing from that falls under this category.   
  
% creating unconnected components: Sometimes two unrelated entities are joined by a relationship .Those errors come under this category of pitfall.

%\textbf{Accuracy Criteria:}The logical inferences drawn from the statements of ontologies should be in accordance of the affairs of the real world.If it fails in doing that then there are flaws in designing of the ontologies.


%Extending the \textit{Accuracy Criteria} an ontology should be able to answer the competency questions which indicates that the ontology fulfills its basic requirements.\cite{ren_towards_2014}.Answering the questions have become one of the 



%In this paper we are proposing an approach that will evaluate ontologies against these established evaluating criterions and will propose alternatives that can help the designer to build better ontologies.
           
%  Ontology Not available: failing to provide online description when looking up its URI.Example is URI not available online as RDF or HTML.
  
%  Several Classes with the Same Label:Like Theatre: both literary discipline and building


==> OntoSeer - A Recommendation System to Improve the Quality of Ontologies /files/Evaluation.tex <==
\section{User Study}
We evaluated OntoSeer through user study by considering the following questions.
\begin{enumerate}
    \item Is OntoSeer useful for the inexperienced as well as the experienced ontology developer? 
    \item Is OntoSeer saving the time of ontology developers?
    \item Are ontology developers able to make richer ontologies due to the axiom recommendations of OntoSeer?
    \item Are the ontology developers reusing existing ontologies more than they generally do?
    \item How easy is it to install and use OntoSeer? 
    \item Are the ontology developers able to create modular ontologies by incorporating ODPs?
    \item Are the ontology developers able to build ontologies that follow the naming conventions?
\end{enumerate}

%\subsection{User Study}

We advertised OntoSeer across several relevant mailing lists\footnote{Prot\'eg\'e users, ODP users, Semantic Web, OWL API} and contacted some of the research groups that work on ontology design. We requested them to use OntoSeer and provide an anonymous response to a questionnaire\footnote{\url{https://github.com/kracr/ontoseer/blob/master/Evaluation/User\%20Study/User\%20Study\%20Questions.txt}}. It had questions on the modelling experience of the users, their familiarity with ODPs, the ease of installing OntoSeer, the relevance of the recommendations provided by OntoSeer, the modelling experience with and without using OntoSeer and whether OntoSeer helps in saving modelling time. 

%\begin{enumerate}
%    \item 
%        How experienced are you with ontology modelling?
%    \item
%    How experienced are you with using Prot\'eg\'e?
%    \item
%      Do you know about LOV and ontology repositories such as BioPortal?
%    \item
%    If Yes, please specify how often do you reuse classes and properties from LOV and ontology repositories?
%    \item 
%    Do you use Ontology Design Patterns (ODPs)?
%    \item
%        If Yes, please specify how often do you use ODPs?
%    \item
%        This section should be answered only if competency questions have been provided to OntoSeer.
%        \begin{enumerate}
%        \item
%            How useful are the class and property recommendations?
%        \item
%            How useful are the ontology vocabulary recommendations?
%        \item
%            How useful are the ODP recommendations?
%        \item
%            How useful are the axiom recommendations?
%        \end{enumerate}
%    \item This section should be answered only if competency questions are not provided to OntoSeer.
%        \begin{enumerate}
%            \item How useful are the Ontology vocabulary recommendations?
%            \item How useful are the ODP recommendations?
%            \item How useful are the axiom recommendations?
%        \end{enumerate}
%    \item How useful is the naming convention checker? 
%    \item How happy are you with the class hierarchy validation?
%    \item How was the installation process?
%    \item How was your experience of modelling an ontology without OntoSeer?
%    \item How was your experience of modelling an ontology with OntoSeer?
%    \item Does Ontoseer help in saving modelling time? 
%    \item Do you have any suggestions for improving the user experience?
%\end{enumerate}

There were 21 respondents. Of the 21 users, 12 have identified themselves as having basic proficiency in Prot\'eg\'e, 7 are at intermediate level and 2 have advanced proficiency in ontology modelling. For evaluating OntoSeer, users can either build an ontology or import an existing ontology. 

%Hence our analysis of OntoSeer's utility for the users with advanced proficiency may not be accurate provide a clear picture but can be used to identify the nature of the trend.

%The users were asked to validate the recommendations from OntoSeer on those ontologies. In this phase of evaluation, users were asked to rate the recommendations of OntoSeer on a scale of 1 to 5, one being the lowest five the highest. The survey has been conducted through an anonymous Google form. The google form for the survey is available at \url{https://github.com/kracr/ontoseer}.

12 users said that the plugin's installation is easy, and the instructions were clear, whereas 7 users found it moderately difficult to install the plugin. Table~\ref{tab:Table5} represents the cumulative user response for vocabulary, ODP and axiom recommendation when the CQs are provided. Table~\ref{tab:Table6} represents the cumulative user response for the same features without the CQs. The ratings are on a scale of 1 to 5, with 1 being the lowest (not satisfied) and 5 is the highest (very satisfied).

\begin{table}[ht] 
\begin{center}
\caption{Average satisfactory index of users for OntoSeer features without CQs}
\label{tab:Table6}
\begin{tabular}{ cccccc } 
 \hline
 Proficiency & Vocabulary & ODP & Axiom  \\ 
 Type  & Recommendation & Recommendation & Recommendation \\
 \hline\hline
 Basic & 4 & 3.67 &4\\ 
 Intermediate & 3.571 &3.571 &3.714\\ 
 Advanced& 3 &3.5 &3\\
 \hline
\end{tabular}
\end{center}
\end{table}

Figures~\ref{fig:tableA} to \ref{fig:ClassHierarchy} are the graphical representations of the user response for the different features of OntoSeer. The average user satisfaction index for name recommendation and class hierarchy validation is given in Table~\ref{tab:Table7}. On an average, users are happy with Ontoseer's recommendations.  Table~\ref{tab:Table5} and Table~\ref{tab:Table6} show that the average satisfaction of users decreases minimally when the intermediate user response is compared with the basic user response (advanced user response is not considered significant since there were only two users). With more modelling experience, users become aware of LOV and ODPs. But even for experienced modellers, OntoSeer can provide useful recommendations. Table~\ref{tab:Table5} and Table~\ref{tab:Table6} also show that the recommendations are better when CQs are available which is an expected result. But the performance of OntoSeer does not drop drastically in the absence of CQs.

%This is predominantly for the users who were installing the plugin in MAC OS.

\begin{table}[ht] 
\begin{center}
\caption{Average satisfactory index of users for OntoSeer features with CQs}
\label{tab:Table5}
\begin{tabular}{ cccc} 
 \hline
 Proficiency & Vocabulary & ODP & Axiom  \\ [0.1ex]
 Type  & Recommendation & Recommendation & Recommendation \\ [0.1ex]
 \hline\hline
 Basic & 4.25 & 4 &4.083\\ 
 Intermediate & 3.86 &3.86 &4.143\\ 
 Advanced& 3 &3.5 &3.5\\
 \hline
\end{tabular}
\end{center}
\end{table}


\begin{table}[ht] 
\begin{center}
 \caption{Average user satisfactory index for OntoSeer's naming recommendation and class hierarchy validation}
\label{tab:Table7}
\begin{tabular}{ ccc } 
 \hline
 Proficiency & Naming  & Class Hierarchy  \\
 Type & Recommendation & Validation \\
 \hline\hline
 Basic & 4.08 & 3.92\\ 
 Intermediate & 4.14 &4\\ 
 Advanced& 4 &3.5 \\
 \hline

\end{tabular}
\end{center}
\end{table}

\begin{figure}[ht]
\centering
  \begin{tabular}{cc}
    \includegraphics[width=0.5\textwidth]{UserStudyResponses/Vocabulary_withCQs.png} &
    \includegraphics[width=0.5\textwidth]{UserStudyResponses/Vocab_withoutCQs.png} 
\end{tabular}
  \caption{User response on the vocabulary recommendation with and without CQs}
  \label{fig:tableA}
\end{figure}

\begin{figure}[htb]
\centering
  \begin{tabular}{cc}
    \includegraphics[width=0.5\textwidth]{UserStudyResponses/Axiom_withCQs.png} &
    \includegraphics[width=0.5\textwidth]{UserStudyResponses/Axiom_withoutCQs.png} 
 \end{tabular}
  \caption{User response on the axiom recommendation with and without CQs}
  \label{fig:tableB}
\end{figure}

\begin{figure}[htb]
\centering
  \begin{tabular}{cc}
    \includegraphics[width=0.5\textwidth]{UserStudyResponses/ODP_withCQs.png} &
    \includegraphics[width=0.5\textwidth]{UserStudyResponses/ODP_withoutCQs.png} 
 \end{tabular}
  \caption{User response on the ODP recommendation with and without CQs}
  \label{fig:tableD}
\end{figure}

\begin{figure}[htb]

 \centering 
\includegraphics[width=10cm, height=5cm]{UserStudyResponses/naming_con.png}
\caption{User response on the name recommendation}
\label{fig:Naming}

\end{figure}

\begin{figure}[htb]

 \centering 
\includegraphics[width=10cm, height=5cm]{UserStudyResponses/ClassHierarchyValidation.png}
\caption{User response on the class hierarchy validation}
\label{fig:ClassHierarchy}
\end{figure}

An important aspect in the evaluation of OntoSeer is the quality of ontology that gets developed and the amount of effort in terms of the time taken to develop an ontology. On average, there is an 8.33\% improvement in modelling experience for the basic proficiency level users when using OntoSeer. This increases to 25.72\% for intermediate proficiency level users. The two advanced proficiency level users chose to be neutral. Fourteen, that is, 66.67\% of users believed that OntoSeer saves modelling time while the remaining seven chose to be neutral (Figure~\ref{fig:ModellingTime}). 

%shows the user response performance of Prot\'eg\'e with OntoSeer over Prot\'eg\'e without OntoSeer concerning modelling time.

%but like the other two groups of users, both of them said that OntoSeer can save significant modeling time.

\begin{figure}[htb]
\centering
  \begin{tabular}{cc}
  \label{fig:table D}
    \includegraphics[width=0.5\textwidth]{UserStudyResponses/OntoWithout.png} &
    \includegraphics[width=0.5\textwidth]{UserStudyResponses/Onto.png} 
\end{tabular}
  \caption{Overall user satisfaction in building ontologies without OntoSeer and with OntoSeer}
\end{figure}


\begin{figure}[htb]

 \centering 
\includegraphics[width=9cm, height=4cm]{UserStudyResponses/OntoSeer_ModellingTime.png}
\caption{User response to the question on whether OntoSeer saves modelling time}
\label{fig:ModellingTime}

\end{figure}

==> OntoSeer - A Recommendation System to Improve the Quality of Ontologies /files/Evaluation_Precision.tex <==
\section{Evaluating the quality of OntoSeer's recommendations}

Using the user study, we evaluated the utility and the effectiveness of OntoSeer's recommendations in real-time, i.e., when it was used as a plug-in while building an ontology in Prot\'eg\'e. There exists the possibility of a bias here because the recommendations were already provided by OntoSeer and the users were asked to evaluate them. In order to avoid this, we evaluate OntoSeer against the users' recommendations, i.e., we first ask the users to make the recommendations which are then compared with OntoSeer's recommendations. We provide two simple use cases in the form of English language descriptions. Along with the descriptions, a few ontologies and ODPs are also provided. Among them, some are relevant to the use case and some are not. Four users were asked to build an ontology (without OntoSeer) by going over each use case and reusing the classes, properties, axioms from the provided ontologies and ODPs. Users worked individually and also in a group of two while building ontologies for the two use cases. The ontologies built by the users, along with the reused classes, properties, axioms from the provided ontologies and ODPs were collected. OntoSeer is then run on the same ontologies and it's recommendations are compared against the ones from the users. In order to mitigate the effects of building the ontologies individually and in a group, we took the union of the recommendations for each use case and compared them with OntoSeer's recommendations. We made these comparisons in two settings. In the exact setting, OntoSeer used only the ontologies and the ODPs provided to the users in order to produce the recommendations. In the general setting, OntoSeer used the entire repository of ontologies and ODPs that were available to it in order to generate the recommendations. Table~\ref{tab:Table17} and Table~\ref{tab:Table18} show the precision and recall of OntoSeer for the use cases 1 and 2 in the general setting. Table~\ref{tab:Table19} and Table~\ref{tab:Table20} show the precision and recall of OntoSeer in the exact setting. From this evaluation, it is evident that OntoSeer's recommendations are relevant and are of good quality. The use cases with all the owl files and user response are available at \url{https://github.com/kracr/ontoseer/tree/master/Evaluation}. 

%The Axiom recommendations in the general scenario will get better with the indexing of more ontologies. %We surveyed 4 users to assess the quality of recommendations provided by OntoSeer by providing the users with two use cases, the first one on online gaming and the second one on book article citation. Along with the use cases, the users were also provided with a few ontologies and ODP, both correct and noisy ones, which they can use for developing the ontologies. The users were asked to build ontologies on these cases without using OntoSeer. The users worked individually and also in a group of 2. To calculate the precision and recall, we took the union of ontologies, ODPs, and axioms used by the users to build the ontologies in both the group and the individual phase as the relevant ones.    

%We validated the recommendations from OntoSeer on these ontologies in both general settings, when OntoSeer has access to all the ODPs and ontologies and in the exact scenario where OntoSeer only has access to the ontologies and ODPs marked relevant by the users.  Table~\ref{tab:Table17} and Table~\ref{tab:Table18} show the average precision and recall recommendations from OntoSeer for the use cases 1 and 2 in the general settings at different k values of 3, 5, and 7, whereas Table~\ref{tab:Table19} and Table~\ref{tab:Table20} shows the precision and recall of recommendations from OntoSeer in the exact scenario. The use cases with all the owl files and user response are available at \url{https://github.com/kracr/ontoseer/tree/master/Evaluation}

%From the Tables, it is evident that OntoSeer recommendations are good even in the general setting. The Axiom recommendations in the general scenario will get better with the indexing of more ontologies.




\begin{table}[ht] 
\begin{center}
 \caption{Precision and recall of OntoSeer for use case 1 in the general setting.}
\label{tab:Table17}
\begin{tabular}{ ccccccc } 
 \hline
Feature&Precision@3 & Recall@3 & Precision@5 & Recall@5 & Precison@7& Recall@7\\
 
 \hline\hline
 ODP&0.66&0.4 &0.6&0.6&0.714 &1\\ 
 Vocabularies&0.66&0.33&0.6&0.5&0.714&0.833\\ 
 Axioms&0.33&0.2&0.4&0.4&0.43&0.6\\
 \hline



\end{tabular}
\end{center}
\end{table}

\begin{table}[ht] 
\begin{center}
 \caption{Precision and recall of OntoSeer for use case 2 in the general setting.}
\label{tab:Table18}
\begin{tabular}{ ccccccc } 
 \hline
Feature&Precision@3 & Recall@3 & Precision@5 & Recall@5 & Precison@7& Recall@7\\
 

 \hline\hline
 ODP&0.33&0.2 &0.6&0.6&0.714 &0.8\\ 
 Vocabularies&0.66&0.4&0.4&0.4&0.571&0.66\\ 
 Axioms&0.33&0.166&0.4&0.33&0.29&0.5\\
 \hline



\end{tabular}
\end{center}
\end{table}

\begin{table}[htb] 
\begin{center}
 \caption{Precision and recall of OntoSeer for use case 1 in the exact setting.}
\label{tab:Table19}
\begin{tabular}{ ccccccc } 
 \hline
Feature&Precision@3 & Recall@3 & Precision@5 & Recall@5 & Precison@7 & Recall@7\\
 
 \hline\hline
 ODP&0.66&0.4 &0.8&0.8&0.714 &1\\ 
 Vocabularies&0.66&0.33&0.66&0.66&0.857&1\\ 
 Axioms&0.66&0.4&0.6&0.6&0.571&0.8\\
 \hline

\end{tabular}
\end{center}
\end{table}

\begin{table}[ht] 
\begin{center}
 \caption{Precision and recall of OntoSeer for use case 2 in the exact setting.}
\label{tab:Table20}
\begin{tabular}{ ccccccc } 
 \hline
Feature&Precision@3 & Recall@3 & Precision@5 & Recall@5 & Precison@7 & Recall@7\\
 
 \hline\hline
 ODP&0.66&0.4 &0.8&0.8&0.571 &0.8\\ 
 Vocabularies&0.66&0.4&0.8&0.8&0.71&1\\ 
 Axioms&0.66&0.33&0.6&0.5&0.71&0.83\\
 \hline

\end{tabular}
\end{center}
\end{table}

==> OntoSeer - A Recommendation System to Improve the Quality of Ontologies /files/RelatedWork.tex <==
\section{Related Work}

Ontology development process involves a series of tasks that are iterative in nature and there is no fixed order for most of the tasks~\cite{article23}. Although there is no one \emph{correct} way of building an ontology, the broad tasks involved in ontology development are as follows. %one needs to carry out for building ontologies. However, it does not imply any execution order instead of the activities that need to be completed. 

\begin{itemize}
    \item List a few competency questions to restrict the scope of the ontology.
    \item Gather the most important terms in the domain.
    \item Split the terms into nouns and verbs. Nouns generally become the classes and verbs become the properties.
    \item Carefully go over the classes and build a hierarchy. The more general classes can be considered as superclasses and the more specific ones become the subclass.
    \item Reuse existing ontologies as much as possible.
    \item The relationship between the concepts should be captured using the axioms.
    \item Appropriate object and data properties should be associated with the classes.
    \item Check whether the ontology can answer the competency questions and if it does not, revise the ontology and repeat some of the listed steps.
\end{itemize}

Each of the above listed steps is subjective and can lead to confusion among the ontology developers. Having the support of a tool in handling these tasks would immensely help the ontology developers. Apart from OntoSeer, there have been a few efforts in this direction. 

Tools that are similar to OntoSeer are  OntoCheck~\cite{DBLP:journals/biomedsem/SchoberTSB12}, and OOPS!~\cite{poveda-villalon_oops!_2014}. We briefly discuss the functionality of these tools and how they differ from OntoSeer.
OntoCheck~\cite{DBLP:journals/biomedsem/SchoberTSB12} is a plugin for Protégé that only indicates the class names that violate the naming convention. For example, if there are classes such as \texttt{HumanBeing}, and  \texttt{nitrogenoxide}, then OntoCheck reports that 50\% of the classes do not follow naming conventions along with the class \texttt{nitrogenoxide}. In contrast, OntoSeer indicates the violation and recommends possible class names such as \texttt{NitrogenOxide} to the user.

OOPS! stands for Ontology Pitfall Scanner. It is an online tool that detects pitfalls or common modelling errors that ontology developers make. The pitfalls are divided into three categories - structural, functional, and usability-profiling. There are around 40 pitfalls, but here we discuss only some of them due to lack of space. Having cycles in the class hierarchy is a pitfall that comes under the structural dimension. Generally, the ontology should not contain more than one semantically equivalent class. Missing disjoint axioms is a common pitfall. Unless explicitly stated, classes are not disjoint. A functional pitfall is connecting disconnected components. Sometimes two unrelated entities are joined by a relationship. This is a pitfall that should be avoided. A usability pitfall is using different naming conventions in the ontology. For example, a superclass will have a name following one naming convention, and a subclass name follows a different naming convention. Missing domain and range for properties is another common pitfall. 

OntoClean~\cite{guarino_overview_2009} provides guidelines for properties and class hierarchies. It introduced terms such as essence, rigidity, identity, and unity. A property that holds in all possible cases is termed as essential for the entity. Rigidity is a type of essential property that is true for all the instances of an entity. A rigid class is a class whose every member cannot cease to be a member without losing its existence. A rigid class cannot be a subclass of an anti-rigid one. Identity is defined as the ability to differentiate two individual entities as different or recognize them as the same. Identity helps in resolving confusion regarding class hierarchies. Unity determines whether an instance is the whole or part of an entity. ODEClean plug-in of WebODE~\cite{DBLP:conf/eon/Fernandez-Lopez02} devised a way to validate class hierarchy with OntoClean taxonomy. Unlike OntoSeer, ODEClean is a stand-alone web plugin.  Also, ODEClean assumes that the user will know the characteristics of each property which may not be true in the case of novice developers. OntoSeer, on the other hand, asks the user simple questions, and based on the answers, validates the class hierarchy.

One of the main differences between OntoClean, OOPS! and OntoSeer is that OntoSeer works along with the ontology developer in creating better quality ontologies. It does not evaluate ontologies post creation. Another major difference is that OntoSeer recommends terms (classes, properties, instances) that can be reused. It does this by checking the similarity of the terms from the ontology being built with existing ontologies. %OntoSeer also recommends ODPs that can be used in making the ontology modular.

An important functionality of OntoSeer is to encourage reusability by making use of existing ontologies and ODPs.  An ODP helps domain experts in ontology engineering by packaging reusable best practices into small blocks of ontology functionality~\cite{DBLP:conf/semweb/Hammar12}. Since there are several hundred ODPs, it is difficult to select the relevant ones. OntoSeer helps users in the selection of ODPs by making use of the classes and properties of the ontology under construction and asking a  few simple questions to the user. This feature is one of major differences between existing tools (described earlier) and OntoSeer.

%The methodology followed in the ODP recommendation is described in section 2.4.

%The ontology requirement specification document can act as a stepping stone for the building of an ontology. Noy and McGuinness in their paper Ontology101~\cite{noy_ontology_2001}, emphasized some fundamental rules in ontology design.
%\begin{enumerate}
%\item There is no one ``correct" way to develop an ontology. There are always viable alternatives. The best solution depends on the application, and the user
%\item Ontology development follows an iterative process.
%\item Concepts in the ontology should be close to objects (physical or logical) and relationships in the domain of interest. These are most likely to be nouns (objects) or verbs (relationships) in sentences that describe the domain.
%\end{enumerate}

%Our tool OntoSeer is compatible with any of the modelling methods undertaken by the developer. The developer, at any point, can change the design, and OntoSeer will update itself accordingly. For a new developer, it is not always possible to determine the scope of the model at first or to have the competency questions. OntoSeer also takes this unfavorable situation into account and provides a recommendation, though better and more refined recommendations will require more prior knowledge of the domain.


%This is from demo paper
%Tools that are similar to OntoSeer are  OntoCheck~\cite{DBLP:journals/biomedsem/SchoberTSB12}, and OOPS!~\cite{poveda-villalon_oops!_2014}. We briefly discuss the functionality of these tools and how they differ from OntoSeer.
%OntoCheck~\cite{DBLP:journals/biomedsem/SchoberTSB12} is a plugin for Protégé that only indicates the class names that violate the naming convention. For example, if there are classes such as ``HumanBeing'', and  ``nitrogenoxide'', then OntoCheck reports that 50\% of the classes do not follow naming conventions along with the class ``nitrogenoxide''. In contrast, OntoSeer indicates the violation and recommends class names such as ``NitrogenOxide'' to the user.

%OOPS! is an online tool that detects pitfalls or common modelling errors that ontology developers make. There are around 40 pitfalls divided into three categories - structural, functional, and usability-profiling. Missing disjointedness axioms is a common pitfall. Unless explicitly stated, classes, are not disjointed. One of the main differences between OOPS! and OntoSeer is that OntoSeer also recommends terms (classes, properties, instances) that can be reused. Apart from that, OntoSeer also recommends ODPs that can be used in making the ontology modular.

%Demo paper related work ends



%This part is left for check whether to add or not.




